PRISM: An Agentic Multi-Model Architecture for Proactive Safety in Autonomous Transportation Systems

Autonomous and intelligent transportation systems operate in complex urban environments where safety depends on interactions among vehicle behavior, environmental conditions, and vulnerable road users (VRUs) such as pedestrians and cyclists. Most advanced driver assistance systems (ADAS) employ reactive mechanisms that activate only after hazards have emerged, a critical limitation underscored by rising VRU fatalities in the United States. This study introduces PRISM (Proactive Risk Intelligence and Safety Management), an agentic multi-model safety architecture that transitions from reactive crash avoidance to proactive, continuous risk management. PRISM employs inverse crash-probability modeling to convert binary crash classifiers into dynamic, interpretable safety scores. Three specialized models addressing trajectory kinematics, environmental risk, and VRU interaction operate concurrently, coordinated by a reasoning layer incorporating reinforcement learning, contextual memory, and feature-level attribution. The system provides graduated safety interventions across four tiers, from silent monitoring to emergency alerts. Unlike rule-based systems with static thresholds, PRISM dynamically adjusts safety parameters in real time. Validated across 1,296 scenarios from three naturalistic driving datasets without dataset-specific retraining, the system yielded a mean safety score of 68 out of 100, classified 77.6% of scenarios as advisory, and flagged a near-miss rate of 3.8%, with 11% of scenarios escalating to intervention or emergency response. Feature attribution consistently identified trajectory risk and VRU proximity as primary safety factors. PRISM provides a unified, interpretable framework for proactive transportation safety with emphasis on VRU risk reduction in dense urban environments.

==> Tables/T7_Intervention_Tier_Distribution.tex <==
\begin{table}[ht]
\centering
\caption{Intervention tier distribution across all three datasets (counts \& \%).}
\label{tab:tiers}
\small
\begin{tabular}{l rr !{\color{gray!50}\vrule} rr !{\color{gray!50}\vrule} rr}
\hline
\textbf{Tier} & \multicolumn{2}{c!{\color{gray!50}\vrule}}{\textbf{nuScenes (n=10)}} & \multicolumn{2}{c!{\color{gray!50}\vrule}}{\textbf{Argoverse 2 (n=1,000)}} & \multicolumn{2}{c}{\textbf{Waymo (n=286)}} \\
 & \textit{n} & \textit{\%} & \textit{n} & \textit{\%} & \textit{n} & \textit{\%} \\
\hline
Emergency    & 2  & 20.0 &  46 &  4.6 &  13 &  4.5 \\
Intervention & 0  &  0.0 &  61 &  6.1 &  18 &  6.3 \\
Advisory     & 7  & 70.0 & 767 & 76.7 & 222 & 77.6 \\
Silent       & 1  & 10.0 & 126 & 12.6 &  33 & 11.5 \\
\hline
\end{tabular}
\end{table}
